A Randomized Approach for Tight Privacy Accounting

Bounding privacy leakage over compositions, i.e., privacy accounting, is a key challenge in differential privacy (DP). The privacy parameter ($\eps$ or $\delta$) is often easy to estimate but hard to bound. In this paper, we propose a new differential privacy paradigm called estimate-verify-release (EVR), which addresses the challenges of providing a strict upper bound for privacy parameter in DP compositions by converting an estimate of privacy parameter into a formal guarantee. The EVR paradigm first estimates the privacy parameter of a mechanism, then verifies whether it meets this guarantee, and finally releases the query output based on the verification result. The core component of the EVR is privacy verification. We develop a randomized privacy verifier using Monte Carlo (MC) technique. Furthermore, we propose an MC-based DP accountant that outperforms existing DP accounting techniques in terms of accuracy and efficiency. Our empirical evaluation shows the newly proposed EVR paradigm improves the utility-privacy tradeoff for privacy-preserving machine learning.

==> appen_PrivUtil_new.tex <==
\privguarantee*


\begin{proof}
We denote event $A = ``\M \text{ is }(\eps, \propdelta+\Delta)\text{-DP}"$ and indicator variable $B = I[\dpv(\M, (\eps, \propdelta), \Delta) = \true]$. Thus, we know that $\fp_\dpv(\M, \eps, \propdelta) = \Pr[B=1 | \bar A]$ and $\tp_\dpv(\M, \eps, \propdelta) = \Pr[B=1 | A]$. For notation simplicity, we denote $\pfp := \fp_\dpv(\M, \eps, \propdelta)$, and $\ptp := \tp_\dpv(\M, \eps, \propdelta)$. 

For any possible set $S$, 
\begin{align}
    &\Pr_{\Maug} \left[ \Maug(D) \in S \right] \nonumber \\ 
    &= \Pr_{\M}[\M(D) \in S | B=1] \Pr[B=1] + 
    I[\reject \in S] \Pr[B=0] \nonumber \\
    &= \Pr_{\M}[\M(D) \in S | B=1, A] \Pr[B=1 | A] I[A] + \Pr_{\M}[\M(D) \in S | B=1, \bar A] \Pr[B=1 | \bar A] I[\bar A] \nonumber \\
    &~~~~+ I[\reject \in S] \Pr[B=0] \nonumber \\
    &\le \left( e^\eps \Pr_{\M}[\M(D') \in S | B=1, A] + \propdelta + \Delta \right) \Pr[B=1 | A] I[A] + \Pr_{\M}[\M(D) \in S | B=1, \bar A] \Pr[B=1 | \bar A] I[\bar A] \nonumber \\
    &~~~~+ I[\reject \in S] \Pr[B=0] \nonumber \\
    &\le \left(e^\eps \Pr_{\M}[\M(D') \in S | B=1, A] + \propdelta  + \Delta \right) \ptp I[A] + \pfp I[\bar A] + I[\reject \in S] \Pr[B=0] \nonumber \\
    &\le e^\eps \left( \Pr_{\M}[\M(D') \in S | B=1, A] \ptp I[A] + \Pr_{\M}[\M(D’) \in S | B=1, \bar A] \pfp I[\bar A] + I[\reject \in S] \Pr[B=0] \right) \nonumber \\
    &~~~~~~+ (\propdelta+\Delta) \ptp I[A] + \pfp I[\bar A] \nonumber \\
    &\le e^\eps \Pr_{\Maug} \left[ \Maug(D') \in S \right] + \max((\propdelta+\Delta) \ptp, \pfp) \nonumber
\end{align}
Therefore, $\Maug$ is $\left(\eps, \max((\propdelta+\Delta) \ptp, \pfp)\right)$-DP. 
By assumption, we have $\pfp \le \propdelta+\Delta$, we know that $\Maug$ is $(\eps, \propdelta+\Delta)$-DP. 
\end{proof}



==> appen_SampleComplexity.tex <==
To show the sample complexity for achieving a DP verifier with target false positive rate, we use a version of Bernstein inequality that is somewhat more general than the classical form of Bernstein’s inequality. 

\begin{theorem}[Generalized Bernstein’s inequality]
\label{thm:bernstein}
Let $X_1, \ldots, X_n$ be independent real valued random variables. Assume that there exist positive numbers $v$ and $c$ such that $\sum_{i=1}^n \E\left[X_i^2\right] \leq v$ and
\begin{align}
\sum_{i=1}^n \E\left[\left(X_i\right)_{+}^q\right] \leq \frac{q !}{2} v c^{q-2} \quad \text { for all integers } q \geq 3.~~~~~~\text{(Bernstein Condition)}
\label{cond:bernstein}
\end{align}
If $S=\sum_{i=1}^n\left(X_i-\E [X_i]\right)$, then for all $\lambda \in (0, 1/c)$ and $t>0$,
$$
\psi_S(\lambda) \leq \frac{v \lambda^2}{2(1-c \lambda)}
$$
and
$$
\psi_S^*(t) \geq \frac{v}{c^2} h\left(\frac{c t}{v}\right),
$$
where $\psi_S(\lambda) := \log (\E[e^{\lambda S}])$ is the cumulant generating function, $\psi_S^*(\lambda) := \sup_{\lambda \in (0, 1/c)} (\lambda t - \psi_S(\lambda))$ the Legendre transform of $\psi_S$, and $h(u) := 1+u-\sqrt{1 + 2u}$ for $u>0$.  
\end{theorem}


\paragraph{Simple Monte Carlo Estimator.}

\begin{restatable}{theorem}{smcsamplecomp}
\label{thm:smc-samplecomp}
    Suppose $\E \left[ \left( \deltamc \right)^2 \right] \le \varbound$. $\mcdpv$ with $\deltamc$ is $(\eps, \delta, \delta)$-guaranteed with 
    $m \ge \frac{1}{ \varbound \left( 1 + \frac{\Delta}{\varbound} - \sqrt{1 + \frac{2\Delta}{\varbound}} \right) } \log(1/\delta)$ samples. 
    Moreover, when $\Delta < \varbound$, we have a more convenient sample complexity $\frac{8 \varbound}{\Delta^2} \log(1/\delta)$. 
\end{restatable}

% \begin{theorem}
%     Suppose $\var \left( \deltamc \right) \le \varbound$. $\mcdpv$ is $(\eps, \delta, \delta)$-guaranteed with 
%     $m \ge \frac{1}{ \varbound \left( 1 + \frac{\Delta}{\varbound} - \sqrt{1 + \frac{2\Delta}{\varbound}} \right) } \log(1/\delta)$ samples. 
%     Moreover, when $\Delta < \varbound$, we have a more convenient sample complexity $\frac{8 \varbound}{\Delta^2} \log(1/\delta)$. 
% \end{theorem}
\begin{proof}

Since $\deltamc$ is a bounded random variable in $[0, 1]$, it is easy to see that the Bernstein condition in (\ref{cond:bernstein}) is satisfied for $\deltamc^m$ with $c=1$. 

\begin{align}
\pfp 
&= \Pr[ \deltamc^m < \deltatilde - \Delta | \deltatilde < \delta ] \\
&\le \Pr[ \deltamc^m < \delta - \Delta | \deltatilde < \delta ] \\
&= \Pr[ \deltamc^m < \delta - \Delta ] \\
&= \Pr \left[ \frac{1}{m} \sum_{i=1}^m (\deltamc^{(i)}-\delta) < -\Delta \right] \\
&= \Pr \left[ \sum_{i=1}^m (\delta-\deltamc^{(i)}) > m\Delta \right] \\
&\le \frac{ \E \left[ \exp\left( m(\delta-\deltamc^{(i)}) \lambda \right) \right] }{ e^{m \Delta \lambda} } \\
&= \exp \left( \log \left( \E \left[ \exp\left( m \lambda (\delta-\deltamc^{(i)}) \right) \right] \right) - m \Delta \lambda \right)
\end{align}
where the second-to-the-last inequality is due to Markov inequality. 

By Theorem \ref{thm:bernstein}, we know that 
\begin{align}
\sup_\lambda \left( m \Delta \lambda - \log \left( \E \left[ \exp\left( m \lambda (\delta-\deltamc^{(i)}) \right) \right] \right) \right) 
&\ge m\varbound h \left( \frac{m\Delta}{m\varbound} \right) \\
&= m\varbound h \left( \frac{\Delta}{\varbound} \right)
\end{align}

Hence,  we have 
\begin{align}
    \pfp \le \exp \left( - m\varbound h \left( \frac{\Delta}{\varbound} \right) \right)
\end{align}

By setting $\exp \left( - m \varbound h \left( \frac{\Delta}{\varbound} \right) \right) \le \delta$, we have
\begin{align}
    m 
    &\ge \frac{1}{ \varbound h \left( \frac{\Delta}{\varbound} \right) } \log(1/\delta) \\
    &= \frac{1}{ \varbound \left( 1 + \frac{\Delta}{\varbound} - \sqrt{1 + \frac{2\Delta}{\varbound}} \right) } \log(1/\delta) 
\end{align}
It is easy to see that the function $h(x) \ge x^2/8$ for $x \in [0, 1]$. Hence, when $\Delta < \varbound$, 
we have
$
\frac{1}{ \varbound \left( 1 + \frac{\Delta}{\varbound} - \sqrt{1 + \frac{2\Delta}{\varbound}} \right) } \log(1/\delta) 
\le 
\frac{8}{ \varbound \left(\frac{\Delta}{\varbound}\right)^2 } \log(1/\delta) 
= \frac{8\varbound}{\Delta^2} \log(1/\delta) 
$. 
\end{proof}


\paragraph{Importance Sampling Estimator: Pure Gaussian}

\issamplecomp*

\begin{proof}
    For pure Gaussian case, since 
    \begin{align}
    \delta 
    &= \E_{t \sim \alterdist} \left[ (1-e^{\eps - t})_+ \frac{\dist(t)}{\alterdist(t)} \right] \\
    &= \E_{t \sim \alterdist} \left[ (1-e^{\eps - t})_+ 
    \frac{M_Y(\theta)}{e^{\theta t}}
    \right]
\end{align}
and for $t \ge \eps$, we have
\begin{align}
    (1-e^{\eps - t})_+ \frac{M_Y(\theta)}{e^{\theta t}} 
    \le \frac{M_Y(\theta)}{e^{\theta \eps}} 
    \le \gamma e^{- \theta \eps}
\end{align}

Moreover, 
\begin{align}
    \E \left[ \left( \deltais \right)^2 \right]
    &= \E_{t \sim \alterdist} \left[ (1-e^{\eps - t})_+^2 \left(\frac{\dist(t)}{\alterdist(t)}\right)^2 \right] \\
    &= \E_{t \sim \dist} \left[ (1-e^{\eps - t})_+^2 \frac{\dist(t)}{\alterdist(t)} \right] \\
    &= \E_{t \sim \dist} \left[ (1-e^{\eps - t})_+^2 \frac{M_Y(\theta)}{e^{\theta t}} \right] \\
    &\le \gamma e^{- \theta \eps} \E_{t \sim \dist} \left[ (1-e^{\eps - t})_+^2  \right] \\
    &\le \gamma \varbound e^{- \theta \eps} 
\end{align}

Hence, the Bernstein condition in Theorem \ref{thm:bernstein} is satisfied by $v := m \gamma \varbound e^{- \theta \eps}$ and $c := \gamma e^{- \theta \eps}$. 
Following a similar derivation as the proof for Theorem \ref{thm:smc-samplecomp}, we have 
\begin{align}
    \pfp \le \exp \left( - \frac{m\varbound}{c} 
    h \left( \frac{\Delta}{\varbound} \right) \right)
\end{align}

By setting $\exp \left( - m \varbound h \left( \frac{\Delta}{\varbound} \right) \right) \le \delta$, we have
\begin{align}
    m 
    &\ge \frac{c}{ \varbound h \left( \frac{\Delta}{\varbound} \right) } \log(1/\delta) \\
    &= \frac{c}{ \varbound \left( 1 + \frac{\Delta}{\varbound} - \sqrt{1 + \frac{2\Delta}{\varbound}} \right) } \log(1/\delta) 
\end{align}
and when $\Delta < \nu$, we have 
$
\frac{c}{ \varbound \left( 1 + \frac{\Delta}{\varbound} - \sqrt{1 + \frac{2\Delta}{\varbound}} \right) } \log(1/\delta) 
\le 
\frac{8c}{ \varbound \left(\frac{\Delta}{\varbound}\right)^2 } \log(1/\delta) 
= \frac{8c\varbound}{\Delta^2} \log(1/\delta) 
= \frac{8\varbound \gamma e^{- \theta \eps} }{\Delta^2} \log(1/\delta) 
$.
\end{proof}

\paragraph{Importance Sampling Estimator: Subsampled Gaussian}
\tianhao{TODO after settling down the IS technique for subsampled Gaussian}




==> appen_hardness.tex <==
\section{Hardness Results for DP Verifier}

\begin{theorem}
    A $\dpv$ with $(\eps, \delta)$-input perfect accuracy (up to certain bits of precision) is \#P-hard. 
\end{theorem}
\begin{proof}
    One can make a reduction from computing the optimal privacy parameters of the composed mechanisms up to $q$ bits to a $\dpv$ with perfect accuracy up to $q$ bits through polynomially many binary searches. By \cite{murtagh2016complexity}, computing the optimal privacy parameters of the composed mechanisms with heterogeneous privacy parameters is \#P-hard, hence  $\dpv$ with perfect accuracy is also \#P-hard. 
\end{proof}

\begin{theorem}
    A deterministic $\dpv$ with dominating pair input requires $O(2^n)$ samples to achieve $(\eps, \delta, \gamma_1, \gamma_2)$-guarantee; a randomized $\dpv$ with dominating pair input requires $O(n)$ samples to achieve $(\eps, \delta, \gamma_1, \gamma_2)$-guarantee. 
\end{theorem}
\begin{proof}
    \tianhao{TODO}
\end{proof}

==> appen_relatedwork.tex <==
An important and active research area in differential privacy is finding the best way to bound the privacy loss under the composition of mechanisms. One approach is to use the discrete Fourier transform of the privacy loss, which involves rounding the privacy loss to a grid. This discretization affects both the accuracy of the final guarantee and the computational efficiency of the computation. While concentrated DP and R'enyi DP use the moment generating function of the privacy loss, these methods instead examine the characteristic function. These techniques offer composition guarantees that are almost optimal and are therefore superior to those obtained through concentrated DP or R'enyi DP.

==> related_work.tex <==
Examples of the existing privacy accounting techniques include the advanced composition theorems \citep{dwork2010boosting}, the moment accountant and R\'enyi differential privacy \citep{abadi2016deep, mironov2017renyi}, convolution and FFT-based methods~\citep{koskela2020computing, koskela2021computing, koskela21a_FFT, gopi2021numerical, ghazi2022faster, doroshenko2022connect}, characteristic function~\citep{zhu2022optimal}, central limit theorem and its finite sample bound \citep{dong2019gaussian, zheng2020sharp, bu2020deep, wang2022analytical}, and saddle-point accountant \cite{alghamdi2022saddle}. 
